Reinforcement Learning based Sequential Batch-sampling for Bayesian Optimal Experimental Design

Engineering problems that are modeled using sophisticated mathematical methods or are characterized by expensive-to-conduct tests or experiments, are encumbered with limited budget or finite computational resources. Moreover, practical scenarios in the industry, impose restrictions, based on logistics and preference, on the manner in which the experiments can be conducted. For example, material supply may enable only a handful of experiments in a single-shot or in the case of computational models one may face significant wait-time based on shared computational resources. In such scenarios, one usually resorts to performing experiments in a manner that allows for maximizing one's state-of-knowledge while satisfying the above mentioned practical constraints. Sequential design of experiments (SDOE) is a popular suite of methods, that has yielded promising results in recent years across different engineering and practical problems. A common strategy, that leverages Bayesian formalism is the Bayesian SDOE, which usually works best in the one-step-ahead or myopic scenario of selecting a single experiment at each step of a sequence of experiments. In this work, we aim to extend the SDOE strategy, to query the experiment or computer code at a batch of inputs. To this end, we leverage deep reinforcement learning (RL) based policy gradient methods, to propose batches of queries that are selected taking into account entire budget in hand. The algorithm retains the sequential nature, inherent in the SDOE, while incorporating elements of reward based on task from the domain of deep RL. A unique capability of the proposed methodology is its ability to be applied to multiple tasks, for example optimization of a function, once its trained. We demonstrate the performance of the proposed algorithm on a synthetic problem, and a challenging high-dimensional engineering problem.

==> conclusions.tex <==
\section{Conclusion}
\label{sec:conclusions}

==> intro.tex <==
\section{Introduction}
\textcolor{red}{Hi Piyush, can you let me know what you think the next steps are for the paper?}\\
\textcolor{blue}{Hi Yonatan, next two steps: polish the intro with solid lit review and two paragrahs on our contributions,
then the methodology explaining our work , basically build upon the stuff you already have in there,
after that , we meet (online or in person) and select the results and conclude.}\\
Design of experiments (DOE) is a field of research ...
\textcolor{blue}{Yonatan, please add a a paragraph on DOE and slowly blend that into the next paragraph about DOE for black-box models.}\\
\textcolor{red}{Do you have the last presentation I made?}

Reinforcement learning has been finding wide application in various fields. 
Molecular optimization, steering optimization in robots, job-shop scheduling, and meta learning to minimize loss functions in machine learning tasks like image classification are some of the areas it has been used \cite{Zhou_2019, robot, andriotis2020deep, li2017learning}. Reinforcement learning(RL) is being widely used because it provides a simple penalty based method to train agents to perform tasks that are hard to optimize otherwise. 
It trains its agents to act effectively in unforeseen environments. 
Complex task environments with large state domains such as those found in the design of experiments are especially well suited for deep RL algorithms.

Design of Experiments (DOE)~\cite{chernoff, bartroff} is an essential aspect of most if not all engineering tasks. 
Tasks ranging from choosing geometric parameters for aircraft rotors to pharmacological drug design require careful experimentation. We want to design our experiments to be reliable, to give useful information, and to be cost effective. These objectives are often taxing and at odds with each other. Smart experimental design effectively addresses these challenges. One important place this is demonstrated is in the optimization of black-box functions that are expensive to evaluate (e.g. to run simulations or lab experiments on the propeller efficiency of rotors with given geometric configurations). 

Querying black-box simulators, that are expensive to evaluate, is an open research problem. 
Bulk of the literature, involves the Bayesian optimization suite of methods~\cite{Jones1998}, that have shown promise in being able to identify the optimal inputs to a simulator with single or multiple objectives.
A Bayesian framework and methodology to optimally design sequential experiments for general non-Gaussian posterior states, and nonlinear forward models (for dynamically defined black-box simulators) has been recently developed by \cite{shen2021}. % mostly amounts to a generalization of state but not necessarily action. They also have an advanced information theoretic reward system. Complimentarily our focus is in action generalization. 
There a design policy that accounts for both feedback and look-ahead design considerations is trained using policy gradient methods of reinforcement learning. 
Nonetheless, a major challenge for BGO methods continues to lie in the practical realm of querying multiple inputs in a single shot.
This task, commonly known as batch sampling,  is motivated by the need of many challenging engineering problems where the overall budget and experimental logistics solicit more than one different inputs. Furthermore, from a theoretical standpoint, the existence of an optimal experimental design for a scenario of a discretized design space with sub-linear relationship between total sample size and design space dimension is unproven. Approximate optimal designs have been shown to exist and have been found for a linear relationship \cite{allen2017}. This points to the imperative of a monotonic relationship been design space dimension and total sample size. Consequently large dimensional engineering problems naturally demand extensive design space sampling that would make batch sampling efficient and cost effective.
Extensions of the classical BGO approach, have shown promise, in alleviating the drawbacks of sub-optimal myopic sampling.
However, the major limitation of these methods that restrict their use in the aforementioned  context are as follows:
a) these methods require a minimum number of inital DOE points in order to train a reliable surrogate model, usually a GP, to being the BGO, and b) the information acquisitions strategies used by these methods do not always account for the long-term expected plausible gains that a batch of points possesses.

The focus of this work, is on optimizing black-box functions, by selecting multiple inputs to query the expensive function. We aim to do this with long term rewards in mind. In other words, we want our algorithm to not be myopic at each sampling step but to optimize the overall effectiveness of the expensive function querying. Deep RL is implemented to meet this challenge. 

Optimizing black box functions using RL has been done using a guided policy search method \cite{li2017learning}. 
The method is designed for searching in large sets of involved policies.
On the other hand, approaches that do not apply machine learning have also been explored. In this paper we combine RL with Gaussian process regression. 
We explore the use of deep RL for sequentially sampling from a black box function and applying a Bayesian Gaussian process regression on the sampled points to find the function's approximate minimal value. 
The state space is a collection of points in the continuous domain of the function and consequently we naturally have a large state domain. 
Hence, the problem is well suited for deep RL methods. 

\textcolor{blue}{Yonatan, please add a paragraph here}
Our main contributions are as follows:
a) Formulating batch sampling for black-box optimization as a task for an RL agent , 
b) Using a parametric policy gradient RL method and nearest neighbor sampling to achieve the aforementioned task,
and, c) Comparing our results with other more familiar methods of batch sampling for Bayesian optimization.

The outline of the document is as follows. In Sec. \ref{sec:metho} we describe the mathematical details of the algorithm developed.
Sec. \ref{sec:results} demonstrate the performance of the methodology on various numerical experiments and comparison with state-of-the-art methods.
In the last section, Sec. \ref{sec:conclusions}, we discuss where our method has potential to outshine previous methods and possibilities for future work.

==> metho.tex <==
\section{Methodology}
\label{sec:metho}
We start with a design space $x=\{x_1,x_2,...,x_n\}$ in $\mathcal{R}^N$ and an objective training function $f(x)$. 
The reinforcement learning system for sequential sampling is modeled as follows:

\begin{enumerate}
    \item \textbf{State($S_i$)}: The sample chosen $Y^{(i)}=\{y^{(i)}_1,y^{(i)}_2,...,y^{(i)}_b\}$ and GP statistics (mean and standard deviation).  
    \item \textbf{Action($A_i$)}: Choose the new sample $Y^{(i+1)}$ in the design space.
    \item \textbf{Reward($r_i$)}: -($\langle y\rangle^{(i)}_{min}-\langle y\rangle^{(i-1)}_{min}+ \alpha(\sigma(y)^{(i)}_{min}-\sigma(y)^{(i-1)}_{min})$)
\end{enumerate}

Here $\alpha$ is the preference parameter between exploration and exploitation in the design space. 
The transition probability distribution is assumed to be unknown. 
This will help with avoiding over-fitting to training function geometry.
We compute the cumulative reward as $R=\sum\limits_{i=1}^{N} \gamma^i r_i$ where $\gamma$ is called the discount factor and is between 0 and 1. When $\gamma$ is small earlier rewards in an episode are prioritized. 
The policy $\pi(a|s)$ gives the probability of taking action a given state s. 

We notice that the system evolution is a partially observable Markov process. 
This prohibits us from resolving the system using dynamic programming methods that use Bellman's equation and by extension the Markov property \cite{sutton}. 
Instead we use REINFORCE the standard policy gradient method. 
The method we use is explained below: 

\textbf{Continuous policy with policy gradient}:
This method uses a normally distributed policy distribution with learn-able parameters. 
Because the policy is differentiable policy we can use policy gradient RL methods to learn the optimal policy for batch sequential sampling for a class of continuous objective functions. 
When our policy model is not differentiable or when the objective is not a continuous function but rather a discrete data set on a mesh-grid we can use "nearest neighbor" approach to modify our policy gradient RL method to overcome the challenge. 
The policy gradient RL method we use throughout is REINFORCE. 
The algorithm is given below:


\begin{algorithm} [H]
\caption{\textbf{REINFORCE for Batch Sequential Sampling}}
\begin{algorithmic}
\item Initialize distribution for the objective function class
\item For i in range (s):
   \item\par \hspace{0.5cm}  Generate sample function $f_i$ from the class of objective functions
    \item\par \hspace{0.5cm} Initialize mesh, episode size(m), number of episodes(n)
    \item\par \hspace{0.5cm} For j in range (n):
         \par\par \hspace{0.5cm} Initialize state (previous batch+ GP statistics), total eps. cost, and storage
         \par\par \hspace{0.5cm} For k in range (m):
         \par\par\par \hspace{1cm} Determine policy for the given state
         \par\par\par \hspace{1cm} Take an sample averaged action from the policy distribution and apply it. 
         \par\par\par \hspace{1cm} Record new state and cost($\langle y\rangle_{min}^k-\langle y\rangle_{min}^{k-1}+\alpha(s_{min}^k-s_{min}^{k-1}) $) in storage
          \par\par\par \hspace{1cm} Update state 
         \par\par \hspace{0.5cm} For k in range (m):
        \par\par\par  \hspace{1cm} Compute cumulative reward from episode step k to m
         \par\par\par \hspace{1cm} Find policy distribution for the state at k
         \par\par\par \hspace{1cm} Update policy WRT cumulative reward.
\end{algorithmic}
\end{algorithm}

We compute the updates for the parameters of the policy distributions for a given episode as follows. 
\begin{equation}
    \begin{aligned}
        &\mu_{i}^{(j)}=\alpha (R[m]-R[j]) (\frac{1}{(\sigma_{i}^{(j)})^2})(ac_{i}-\mu_{i}^{(j)}), \\
        &(\sigma^{(j)}_{i})^2= -0.5\alpha (R[m]-R[j])((\frac{1}{(\sigma_{i}^{(j)})^2}) (ac_{i} - \mu_{i}^{(j)})^2+(\frac{1}{(\sigma_{i}^{(j)})^2}))
    \end{aligned}
\end{equation}
Here $\mu_i^{(j)}$ and $(\sigma_{i}^{(j)})^2$ are the mean and standard deviation of the policy distribution at episode step i. 
$ac_i$ is the action taken by the agent for the state at episode step i and $\alpha$ is the policy learning rate. 

Because the objective function is a black box function on a mesh-grid we add a few more steps. 
First, we take a sample averaged action from the policy distribution. 
That is, we take multiple batches sampling from the policy and average them. 
Then we find the nearest neighbor in our grid file for each sample averaged batch removing points from the grid file as we go. 

==> results.tex <==
\section{Numerical examples}
\label{sec:results}
\label{sec:numerics}
\subsection{Ackley and Booth function}

We consider the problem of inferring statistics of an unknown permeability field along a one-dimensional column that is characterized by a porous medium. 
Such problems are of particular interest in the geoscience community, where the sufficient characterization of the subsurface is often subject to financial costs and therefore, optimal Bayesian decision making strategies need be pursued. 
Studies for characterizing the hydraulic conductivity in realistic subsurface domain settings using such worth-of-information strategies have been extensively presented before \cite{freeze, james_gorelick, tsilifis}. 
This simplified example serves only a motivation for potential applications of the methodology proposed herein. 
